TabFM-Auto: Self-Evolving Pipelines for Tabular Foundation Models

Tabular foundation models achieve strong zero-shot accuracy on structured data by pretraining on synthetic tables, but they ignore the column names, task descriptions, and auxiliary files that carry dataset semantics. Meanwhile, self-evolving machine learning engineering (MLE) agents train models from scratch on each dataset, yet jointly searching over features, architectures, and hyperparameters is noisy and prone to overfitting. We introduce TabFM-Auto, which pairs a tabular foundation model, TabFM, with a language model agent that evolves the data pipeline around it. Guided by dataset metadata and validation feedback, TabFM-Auto iteratively refines data cleaning, feature engineering, context selection, and post-processing to reduce TabFM's error. Across all 51 datasets of the TabArena benchmark, five TabFM-Auto configurations with different agents and language models take the top five overall positions, and the best raises TabFM from 1785 to 2013 Elo. The discovered pipelines also transfer to other frozen tabular foundation models (+69 to +143 Elo) with no further search. On the 8 tabular competitions of MLE-Bench, TabFM-Auto ranks first overall among MLE agents.

==> sections/iclr_statements.tex <==
\clearpage
\section*{AI Use Statement}
In accordance with the ICLR 2027 policy on the use of generative AI, we distinguish between the LLM coding agents that form the empirical subject of our experiments and the generative AI tools used by the authors during the research workflow. As the subject of study, \tabfmauto{} evaluates LLM coding agents (\texttt{Claude Opus 5} and \texttt{Gemini 3.8 Flash} paired with the \texttt{Claude Code}, \texttt{Codex}, and \texttt{Antigravity} harnesses) on their ability to evolve data pipelines (\texttt{preprocess()}, \texttt{engineer()}, \texttt{sample()}, \texttt{postprocess()}, and \texttt{TABFM\_KWARGS}) around frozen tabular foundation models in an isolated evaluation harness. Within the authors' own workflow, we used generative AI tools only to assist with coding and to edit manuscript prose for readability. We did not use generative AI for any other research tasks. All AI-assisted code and text were manually reviewed, tested, and verified for correctness by the authors. We take full responsibility for the final content of this work, including all text, code, claims, and artifacts produced with the aid of generative AI.

\section*{Ethics Statement}
The authors have read and adhere to the ICLR Code of Ethics. All experiments use publicly released, de-identified benchmark datasets (\texttt{TabArena} and \texttt{MLE-Bench}) in accordance with their open-source licenses, without human subjects, crowdworker annotation, or personally identifiable information. Because evaluating coding agents involves executing LLM-generated Python programs, the evaluation harness runs all agent-written code in the network-isolated Linux \texttt{bubblewrap} namespace sandbox described in Section~\ref{sec:method} and Appendix~\ref{sec:app_verification}. This sandbox disables outbound network connections, mounts system libraries and benchmark data read-only, unmounts held-out test splits during search, and restricts writes to an ephemeral scratch directory. While automating data pipeline construction around tabular foundation models lowers the barrier to applying machine learning across scientific and enterprise tables, deploying evolved pipelines in high-stakes domains such as healthcare, finance, or public policy requires domain-specific fairness, calibration, and distribution-shift audits prior to real-world use.

\section*{Reproducibility Statement}
All datasets and official train/test splits evaluated in this work come from two public benchmarks: the 51-dataset TabArena benchmark~\citep{erickson2025tabarena} (3-fold cross-validation repeated 3 or 10 times, see Section~\ref{sec:exp_tabarena}) and the 8 tabular competitions of MLE-Bench~\citep{chan2024mlebench} (official local splits, see Section~\ref{sec:exp_mlebench} and Appendix~\ref{sec:app_mlebench_details}). Section~\ref{sec:method} and Appendix~\ref{sec:app_verification} detail the pipeline search objective in Equation~\eqref{eq:auto_obj}, the five pipeline components (\texttt{preprocess()}, \texttt{engineer()}, \texttt{sample()}, \texttt{postprocess()}, and \texttt{TABFM\_KWARGS}), and the sandboxed evaluation protocol (including the identity baseline check $P_0$, filesystem split isolation, and deterministic row-order permutation). Section~\ref{sec:exp_tabarena} and Appendix~\ref{sec:app_leaderboard_analysis}--Appendix~\ref{sec:app_transfer} specify the Bradley--Terry Elo rating procedure (anchored to Random Forest at 1000 Elo across the 66-method TabArena pool), the single-fold and multi-fold evaluation protocols, the unconstrained coding-agent ablation (Appendix~\ref{sec:app_free_agent}), and the zero-shot pipeline transfer protocol across frozen tabular foundation models (\texttt{TabPFN-3}, \texttt{TabICLv2}, and \texttt{EXAONE-Tabular}). Sections~\ref{sec:exp_tabarena} and~\ref{sec:exp_mlebench} state the search budgets (up to 96 evaluations or 6 hours on one H100 GPU per TabArena dataset and 24 hours per MLE-Bench-Tabular competition), and Table~\ref{tab:token_consumption} reports evaluation counts, token consumption, and tool-invocation distributions. Finally, Figure~\ref{fig:identity_pipeline} lists the starting pipeline $P_0$, and Figure~\ref{fig:fe_case_studies} and Table~\ref{tab:feature_engineering_taxonomy} provide representative evolved Python pipelines and stage-level taxonomy counts, while Tables~\ref{tab:transfer}--\ref{tab:all_51_datasets} report complete transfer and per-dataset official test results across all 59 tasks.

